On-board GRB trigger algorithms of SVOM-GRM

GRM (Gamma-Ray Monitor) is the high energy detector on-board the future Chinese-French satellite SVOM (Space-based multi-band astronomical Variable Object Monitor) which is dedicated to Gamma-Ray Burst (GRB) studies. This paper presents the investigation of the on-board counting rate trigger algorithms of GRM. The trigger threshold and trigger efficiency based on the given GRB sample are calculated with the algorithms. The trigger characteristics of GRM and ECLAIRs are also analyzed. In addition, the impact of solar flares on GRM is estimated, and the method to distinguish solar flares from GRBs is investigated.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

